Few-Shot Learning for Opinion Summarization

Opinion summarization is the automatic creation of text reflecting subjective information expressed in multiple documents, such as user reviews of a product. The task is practically important and has attracted a lot of attention. However, due to the high cost of summary production, datasets large enough for training supervised models are lacking. Instead, the task has been traditionally approached with extractive methods that learn to select text fragments in an unsupervised or weakly-supervised way. Recently, it has been shown that abstractive summaries, potentially more fluent and better at reflecting conflicting information, can also be produced in an unsupervised fashion. However, these models, not being exposed to actual summaries, fail to capture their essential properties. In this work, we show that even a handful of summaries is sufficient to bootstrap generation of the summary text with all expected properties, such as writing style, informativeness, fluency, and sentiment preservation. We start by training a conditional Transformer language model to generate a new product review given other available reviews of the product. The model is also conditioned on review properties that are directly related to summaries; the properties are derived from reviews with no manual effort. In the second stage, we fine-tune a plug-in module that learns to predict property values on a handful of summaries. This lets us switch the generator to the summarization mode. We show on Amazon and Yelp datasets that our approach substantially outperforms previous extractive and abstractive methods in automatic and human evaluation.

==> content/sections/error_analysis.tex <==
% \subsection{Error Analysis}
% We also performed qualitative error analysis of generated summaries, and observed that there are two types of common mistakes. In the first case, the model generates a wrong main entity, such as the name of the brand or product. We believe that this can be improved by using the copy mechanism and pre-trained language models. Second, we observed that the model generates factual incorrect summaries 

% % Generic phrases that can be 

% Wrong entities



==> content/summs/amazon/base_vs_full.tex <==

\begin{wraptable}{c}{6cm}
% \begin{table}[h!]
    \centering
 	\footnotesize 
    \begin{tabular}{ | >{\centering\arraybackslash} m{1cm} | m{5cm} |}
    \hline
    Base & This bag is very cute, but it is a bit smaller than I thought it would be. However, it is still a great bag for the price. \\ \hline
    Full & \\ \hline
    \end{tabular}
    \caption{An example summary produced by our system and human-written one with colored content alignment. The eight input reviews are concatenated and truncated for visibility.}
    \label{table:ama_summ_base_vs_full}
% \end{table}
\end{wraptable}

==> content/summs/yelp/summ1.tex <==
%RqOgBMpKYdsEOmBVmFXe3g

\begin{table*}
    \centering
 	\footnotesize 
    \begin{tabular}{  >{\centering\arraybackslash} m{1.5cm} m{12cm}}
 \thickhline
    Gold & \vspace{0.5em} The menu is vegetarian friendly. Attentive and efficient service. Very unique broth and the toppings are non traditional. The food was amazing and the filling impeccable. The ramen is absolutely outstanding. The bathrooms are cool and the toilet seats are heated.\vspace{0.5em} \\ \hline
    Ours & \vspace{0.5em} This is one of the best ramen restaurants in the city. The broth is very flavourful and the noodles are very flavourful. The ramen is also very good. The staff is very friendly and the restaurant is very clean.\vspace{0.5em} \\ \hline
    Copycat & \vspace{0.5em} This is my favourite ramen place in Toronto. I've tried many of the dishes, but this is one of my favourite places to eat. The staff is super friendly and helpful. I'll definitely be back!\vspace{0.5em}  \\ \hline
    MeanSum & \vspace{0.5em} A little pricey, but the food is delicious. I got a ramen and this was a good size dish! Everything else was fresh. The broth is rich and creamy as well. I'm not a fan of their ramen, but it was a bit pricey for me. Still, I will be back for more. \vspace{0.5em} \\ \hline
    Lexrank & \vspace{0.5em} That is real Japanese ramen!!! One of my favourite ramen places. I had the vegetarian bowl! definitely different approach to ramen.Overall: probably wont be back, ill rather go to kinton down the road. This was my first time trying ramen in the city, and it was a fabulous first experience. \vspace{0.5em} \\ \hline
     \thickhline
    Review 1 & \vspace{0.5em} Atmosphere: located on the famous baldwin street, modern, trendyFood: cold noodles special, 3 / 5, the noodles were legit cold. which was unexpectedly different. definitely different approach to ramen.Overall: probably wont be back, ill rather go to kinton down the road.\vspace{0.5em} \\ \hline
    Review 2 & \vspace{0.5em} This was my first time trying ramen in the city, and it was a fabulous first experience. I have yet to try anything that lived up to this place. The food was delicious and filling, and the service impeccable. Will definitely be back, many many times.\vspace{0.5em} \\ \hline
    Review 3 & \vspace{0.5em}Ryus owner is Japanese and it shows. I tried other ramen restaurants in Toronto but some others are NOT Japanese. These other restaurants do not serve the Japanese style. Please try Ryus Miso ramen. That is real Japanese ramen!!! I love it!!!\vspace{0.5em} \\ \hline
    Review 4 & \vspace{0.5em} One of my favourite ramen places. Broth is so flavourful and when they say spicy, it's spicy. Not the watered down Canadian level of spicy. The service is excellent and free refills on pop, I'll take it.\vspace{0.5em} \\ \hline
    Review 5 & \vspace{0.5em} I'm glad Ryus reopened after the fire which completely destroyed the Baldwin location. I've always been a loyal follower because of their unique broth and the non traditional toppings they use. Plus their menu is very vegetarian friendly. Service is efficient and attentive. This new locale is across from the Broadview station with lots of street parking.\vspace{0.5em} \\ \hline
    Review 6 & \vspace{0.5em} Absolutely outstanding Ramen. Pork blaster 'hot' has to be a personal favourite. Very filling and rich broth and the spice was good enough to excite my Indian palate... That's really saying something! Will definitely return although I can't say I'd try much else since I'm sold on this one dish. Patio is highly recommended! \vspace{0.5em} \\ \hline
    Review 7 & \vspace{0.5em} I had the vegetarian bowl! Yummy, just right for me.. I prefer it to Kinton's veg. bowl. I really like the atmosphere! Service was very nice and attentive, was a great meal to have with some out of town friends. Ps....... Bathrooms are really cool. Toilet seats are heated. Crazy. \vspace{0.5em} \\ \hline
    Review 8 & \vspace{0.5em} It's hard to compete with 'Kinton' a few shops down, but with their prices and original / delicious broths, they are in contention. It's a nice place to go for cheap, fast, and feeling Ramen. They let you choose which oil / sauce you want on the side which is neat.\vspace{0.5em} \\ \thickhline
    \end{tabular}
    \caption{Example summaries produced by different systems on Yelp data.}
\end{table*}

